Weighted Edit Distance Computation: Strings, Trees and Dyck

Given two strings of length $n$ over alphabet $\Sigma$, and an upper bound $k$ on their edit distance, the algorithm of Myers (Algorithmica'86) and Landau and Vishkin (JCSS'88) computes the unweighted string edit distance in $\mathcal{O}(n+k^2)$ time. Till date, it remains the fastest algorithm for exact edit distance computation, and it is optimal under the Strong Exponential Hypothesis (STOC'15). Over the years, this result has inspired many developments, including fast approximation algorithms for string edit distance as well as similar $\tilde{\mathcal{O}}(n+$poly$(k))$-time algorithms for generalizations to tree and Dyck edit distances. Surprisingly, all these results hold only for unweighted instances. While unweighted edit distance is theoretically fundamental, almost all real-world applications require weighted edit distance, where different weights are assigned to different edit operations and may vary with the characters being edited. Given a weight function $w: \Sigma \cup \{\varepsilon \}\times \Sigma \cup \{\varepsilon \} \rightarrow \mathbb{R}_{\ge 0}$ (such that $w(a,a)=0$ and $w(a,b)\ge 1$ for all $a,b\in \Sigma \cup \{\varepsilon\}$ with $a\ne b$), the goal is to find an alignment that minimizes the total weight of edits. Except for the vanilla $\mathcal{O}(n^2)$-time dynamic-programming algorithm and its almost trivial $\mathcal{O}(nk)$-time implementation, none of the aforementioned developments on the unweighted edit distance apply to the weighted variant. In this paper, we propose the first $\mathcal{O}(n+$poly$(k))$-time algorithm that computes weighted string edit distance exactly, thus bridging a fundamental gap between our understanding of unweighted and weighted edit distance. We then generalize this result to weighted tree and Dyck edit distances, which lead to a deterministic algorithm that improves upon the previous work for unweighted tree edit distance.

==> notes.tex <==
\section{8/29}

Parameterized fine grain algorithms:  can we find a $O(n + poly(k))$ algorithm for a wide variety of problems?

Diameter  (see https://arxiv.org/pdf/1802.10048.pdf), APSP, matching

RNA folding has a lower bound such that no such alg exists (Tomasz + Barna old paper idea).

For matching, $O(kn)$ is trivial, can just use an augmenting path algorithm $k$ times.

Define problem as minimum weight of sequence of operations.

Add abstract with triangle inequality weighted versions: start with weighted edit distance, later improve the bounds and remove triangle inequality, generalize to Dyck and forest, first paper with weighted problems (first results, time considered)

- At some point we may want to discuss $k^5$ kernel lowerbounds for weighted edit distance

micro-macro decompositions = contexts & forests

- Jake: Start writing the overview with $O(\min ((n^2), nk))$ folklore for weighted.  Some motivation for problem: unweighted edit distance is a somewhat theoretical problem, in real world we always care about weighted edit distance. While we can get a simple solution for multiplicative edit distance, not the same for tree/dyck.  However, in general, additive is the goal. Holy grail to get additive, so far weighted there is nothing except simple multiplicative edit distance.

Try to write a connection between weighted version & kernelization, and we have some evidence that $k^5$.

For simplicity, we've considered unweighted case.  In real-world, almost always weighted.  In this case, we focus on weighted case, we get the holy-grail. When weights are polynomially small in terms $n$.

In second paragraph of abstract, mention the tools of our paper (periodicity may be useful). Practical tools.

For deadline

Overview:

Strings - corollary of thm that we can solve in $n + k^5$ based on nk

Section 8 - algorithm description, bullet points can be described
- kernel can be used for n + poly(k) ted alg.

- Debarati doing Dyck section

Lemma 12.1 check if proof goes the same

Make sure to emphasize difference from unweighted paper
(need to add a citation) in overview

4 sections + subsections

Similarly to our weighted string edit distance algorithm, in section~\ref{sec:ted} our weighted tree edit distance algorithm identifies synchronized subforests that we would like to find a small edit distance equivalent subforest for.  Again, we begin by showing that the number of repetitions of periodic sections of a forest may be reduced. However, periodicity in forests is a bit less well-defined, and so, we utilize two types of periodicity, \emph{horizontal} and \emph{vertical} periodicity, first proposed by \cite{DGHKSS'22}.  Horizontal $k$-periodicity occurs in forest $F$ when there is a subforest of size at most $4k$ repeated more than $4k$ times. Vertical $k$-periodicity is more complicated than horizontal $k$-periodicity and occurs when there is a path through a forest in which the left half of the path is periodic and the right half of the path is periodic (the halves may have different periods). \jgnote{Going to add a figure for this, perhaps stealing the previous papers' figure} To easily identify these types of periodicity, we consider forests as strings of balanced parentheses (see: Subsection~\ref{subsec:treeprelim}).  Therefore, finding horizontal periodicity reduces to finding maximal balanced periodic substrings, and finding vertical periodicity reduces to finding pairs of maximal periodic substrings that are balanced when concatenated to each other. With these reductions in mind, we give Algorithm~\ref{alg:family_per_reduc}, which is a new useful algorithm that takes an input string $P$, a number $e \in \mathbb{Z}$, and a family of strings $\Qf$ and then outputs a string $R$ that is exactly equal to $P$ excluding any repetitions of a substring in $\Qf$ after $e$ repetitions. The algorithm requires an oracle that can identify whether a substring $Q$ is a member of $\Qf$ in constant time. By defining $\Qf$ to be all substrings representing horizontal and vertical periodicity and providing and providing implementations of the relevant oracles (see Subsection~\ref{subsec:treealg} for details), we can construct edit distance equivalent forests that avoid horizontal and vertical $k$-periodicity.

Once we have avoided horizontal and vertical periodicity, finding small edit distance equivalent forests and contexts is similar to that of strings. In fact for forests and contexts, we prove slightly stronger results. We show that forests of size $\Omega(k^3)$ that avoid horizontal $k$-periodicity are edit distance equivalent, and contexts of size $\Omega(k^4)$ that avoid vertical $k$-periodicity and do not contain balanced substrings of size $\Omega(k^3)$ (we may use our horizontal $k$-periodicity reduction first if so) are edit distance equivalent. These stronger results follow from the added structures present in trees as compared to strings.  An alignment may break a string into two substrings using an edit, but in trees, unless the alignment deletes a root node, the tree is still a single tree.  Therefore, there is always an optimal alignment that will match synchronized occurrences of large forests and contexts exactly, and otherwise, there would be horizontal or vertical $k$-periodicity. Thus, given synchronized occurrences of forests and contexts that avoid periodicity, we may choose any forest of size $O(k^3)$ and context of size $O(k^4)$, respectively, when constructing small instances of edit distance equivalent forests.

==> old_stuff.tex <==

\section{Open Problems}

\begin{enumerate}
\item Unlabeled ordered tree edit distance, is this much easier than labeled?  If so, what about constant alphabet tree edit distance.

\item $O(n + \text{poly($k$)})$ exact tree edit distance solution, potentially improving current best runtime, $O(n k^2 \log n)$.

\item Weighted string edit distance, tree edit distance, Dyck edit distance approximate solutions:
\begin{enumerate}
    \item Costs depending only on operation and label, not position
    \item Costs depending on positions as well
\end{enumerate}

\item Weighted hardness results, extending the APSP reduction for tree edit distance or maybe using orthogonal vector matrix hardness

\item Look into Triangle Inequalities for weighted versions, see where they may hold up, where they may break.
\end{enumerate}
